Estimation and Inference in Distributional Reinforcement Learning

In this paper, we study distributional reinforcement learning from the perspective of statistical efficiency. We investigate distributional policy evaluation, aiming to estimate the complete return distribution (denoted $\eta^\pi$) attained by a given policy $\pi$. We use the certainty-equivalence method to construct our estimator $\hat\eta^\pi$, given a generative model is available. In this circumstance we need a dataset of size $\widetilde O\left(\frac{|\mathcal{S}||\mathcal{A}|}{\varepsilon^{2p}(1-\gamma)^{2p+2}}\right)$ to guarantee the $p$-Wasserstein metric between $\hat\eta^\pi$ and $\eta^\pi$ less than $\varepsilon$ with high probability. This implies the distributional policy evaluation problem can be solved with sample efficiency. Also, we show that under different mild assumptions a dataset of size $\widetilde O\left(\frac{|\mathcal{S}||\mathcal{A}|}{\varepsilon^{2}(1-\gamma)^{4}}\right)$ suffices to ensure the Kolmogorov metric and total variation metric between $\hat\eta^\pi$ and $\eta^\pi$ is below $\varepsilon$ with high probability. Furthermore, we investigate the asymptotic behavior of $\hat\eta^\pi$. We demonstrate that the ``empirical process'' $\sqrt{n}(\hat\eta^\pi-\eta^\pi)$ converges weakly to a Gaussian process in the space of bounded functionals on Lipschitz function class $\ell^\infty(\mathcal{F}_{\text{W}})$, also in the space of bounded functionals on indicator function class $\ell^\infty(\mathcal{F}_{\text{KS}})$ and bounded measurable function class $\ell^\infty(\mathcal{F}_{\text{TV}})$ when some mild conditions hold. Our findings give rise to a unified approach to statistical inference of a wide class of statistical functionals of $\eta^\pi$.

==> asymp_old.tex <==

\subsection{Results on Asymptotic Analysis}\label{Section_asymp}

We first give our main results of asymptotic analysis in Theorem~\ref{Theorem_weak_convergence_empirical_process} and then 
explain it in more details in Section~\ref{sec:analysisofthm2}.

\begin{theorem}\label{Theorem_weak_convergence_empirical_process}
    For any fixed policy $\pi$, we have for any $s\in\gS$
    \begin{enumerate}
        \item[\emph{(a)}] $\sqrt{n}\prn{\hat\eta_n^\pi(s)-\eta^\pi(s)}$ converge weakly to the process $f\mapsto \brk{\prn{\gI-\gT^\pi}^{-1}\wtilde\GB^\pi}(s)f$ in $\ell^\infty(\FLip)$, where $\FLip:=\brc{f\colon f \text{ is supported on $\brk{0,\frac{1}{1-\gamma}}$ and $1$-Lipschitz}}$.
        \item[\emph{(b)}] If Assumption~\ref{Assumption_reward_bounded_density} is true, then $\sqrt{n}\prn{\hat\eta_n^\pi(s)-\eta^\pi(s)}$ converge weakly to the process $f\mapsto \brk{\prn{\gI-\gT^\pi}^{-1}\wtilde\GB^\pi}(s)f$ in $\ell^\infty(\FInd)$, where $\FInd:=\brc{\ind_{(-\infty,z]}\colon  z\in\brk{0,\frac{1}{1-\gamma}}}$.
    \end{enumerate}
    
    Here the random element $\wtilde\GB^\pi$ is defined as
    \begin{equation*}
        \wtilde\GB^\pi(s):=\sum_{a\in\gA}\pi(a\mid s)\sum_{s^\prime\in\gS} Z_{s,a,s^\prime}\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\ \forall s\in\gS,
    \end{equation*}
    where  $\prn{Z_{s,a,s^\prime}}_{s\in\gS,a\in\gA,s^\prime\in\gS}$ are zero-mean gaussians with 
    \begin{equation*}
        \cov(Z_{s_1,a_1,s_1^\prime},Z_{s_2,a_2,s_2^\prime})=\ind\brc{(s_1,a_1)=(s_2,a_2)}P(s_1^\prime\mid s_1,a_1)\prn{\ind\brc{s_1^\prime=s_2^\prime}-P(s_2^\prime\mid s_1,a_1)}.
    \end{equation*}
\end{theorem}

Generally speaking, we depict the asymptotic behavior of $\sqrt{n}\prn{\hat\eta^\pi_n-\eta^\pi}$ by showing that the ``empirical processes" induced by $\sqrt{n}\prn{\hat\eta^\pi_n-\eta^\pi}$ converge to a Gaussian random element.
Moreover, the limiting random element has a simple structure in the sense that it is a finite mixture of probability distributions with Gaussian coefficients.
% And the covariance function can be consistently estimated using standard plug-in approaches (use $\what P$ in place of $P$ and $\hat\eta_n^\pi$ in place of $\eta^\pi$).
Our proof of Theorem~\ref{Theorem_weak_convergence_empirical_process} builds on a careful analysis of the behaviors of the distributional Bellman operator $\gT^\pi$ when extended to the space of signed measures.

\subsubsection{Analysis of Theorem~\ref{Theorem_weak_convergence_empirical_process}}
\label{sec:analysisofthm2}

Before presenting our proofs, we first define some notations.
Given some function class $\gF$ supported on $\brk{0,\frac{1}{1-\gamma}}$, we use $\ell^\infty(\gF)$ to denote the space of bounded real-valued functions on $\gF$.
$\ell^\infty(\gF)$ is a Banach space if we equip it with the supreme norm $\norm{\cdot}_\gF$.
For any signed Borel measure $\mu$, we define $\norm{\mu}_\gF:=\sup_{f\in\gF}\abs{\mu f}$.
We use $M_\gF$ to denote the vector space of signed Borel measures with finite $\norm{\cdot}$ norm, formally, define $\gB_0$ as the Borel sets in $\brk{0,\frac{1}{1-\gamma}}$,
\begin{equation*}
    M_\gF:=\brc{\mu\text{ signed measure on }\prn{\brk{0,\frac{1}{1-\gamma}},\gB_0},\norm{\mu}_\gF<\infty}.
\end{equation*}
Note that $(M_\gF,\norm{\cdot}_\gF)$ can be embedded into $(\ell^\infty(\gF),\norm{\cdot}_\gF)$ by mapping $\mu$ to the process $f\mapsto \mu f$.

The distributional Bellman operator $\gT^\pi$ can be naturally extended to $\prn{M_{\gF}}^\gS$ without modifying its original definition.
Here, the product $\left(M_{\mathcal{F}}\right)^\mathcal{S}$ also constitutes a normed vector space, where the norm is defined as $\sup_{s\in\mathcal{S}}\norm{\cdot}_{\mathcal{F}}$.

\begin{proposition}\label{Proposition_extention_of_Bellman_operator}
    $\gT^\pi$ is a linear operator on $\prn{M_{\gF}}^\gS$.
\end{proposition}

The proof is straightforward by noting the linearity of the push-forward operation.

\paragraph{Weak Convergence in $\ell^\infty(\gF_{\mathsf{Lip}})$}

$M_{\FLip}$ contains all probability measures supported on $\brk{0,\frac{1}{1-\gamma}}$.
Therefore, we have
\begin{equation*}
\begin{aligned}
    \sqrt{n}(\hat\eta_n^\pi-\eta^\pi)&=\sqrt{n}\prn{\what \gT_n^\pi\hat\eta_n^\pi-\gT^\pi\eta^\pi}\\
    &=\sqrt{n}\prn{\what \gT_n^\pi\hat\eta_n^\pi-\what \gT_n^\pi\eta^\pi+\what \gT_n^\pi\eta^\pi-\gT^\pi\eta^\pi}\\
    &=\sqrt{n}\what \gT_n^\pi(\hat\eta_n^\pi-\eta^\pi)+\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi\\
    &=\sqrt{n}\gT^\pi(\hat\eta_n^\pi-\eta^\pi)+\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi+\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi).\\
\end{aligned}
\end{equation*}
Rearranging terms yields
\begin{equation*}
    \sqrt{n}\prn{\gI-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)=\underbrace{\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}_{(1)}+\underbrace{\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}_{(2)}.
\end{equation*}
Next, we can show that term $(1)$ converges weakly to a mixture of probability distributions and term $(2)$ is negligible.
One may refer to Appendix~\ref{Appendix_proof_asymp} for detailed proof.
\begin{lemma}\label{Lemma_convergence_difference_operator}
For any $s\in\gS$, $\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}(s)$ converge weakly to the process $f\mapsto \wtilde\GB^\pi(s)f$ in $\ell^\infty(\FLip)$.
Here the random element $\wtilde\GB^\pi$ is defined as
    \begin{equation*}
        \wtilde\GB^\pi(s):=\sum_{a\in\gA}\pi(a\mid s)\sum_{s^\prime\in\gS} Z_{s,a,s^\prime}\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\ \forall s\in\gS,
    \end{equation*}
    where  $\prn{Z_{s,a,s^\prime}}_{s\in\gS,a\in\gA,s^\prime\in\gS}$ are zero-mean gaussians with 
    \begin{equation*}
    \cov(Z_{s_1,a_1,s_1^\prime},Z_{s_2,a_2,s_2^\prime})=\ind\brc{(s_1,a_1)=(s_2,a_2)}P(s_1^\prime\mid s_1,a_1)\prn{\ind\brc{s_1^\prime=s_2^\prime}-P(s_2^\prime\mid s_1,a_1)}.
    \end{equation*}
\end{lemma}
\begin{lemma}\label{Lemma_convergence_res_op1}
For any $s\in\gS$, we have $\norm{\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}(s)}_{\FLip}=o_P\prn{1}$.
\end{lemma}
Now it remains to relate $\sqrt{n}\prn{\gI-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)$ with $\sqrt{n}\prn{\hat\eta_n^\pi-\eta^\pi}$.
This can be immediately accomplished if $\prn{\gI-\gT^\pi}$ is invertible on $M^\gS$.
The invertibility does not hold since $(\gI-\gT^\pi)$ is a linear operator and has a non-trivial kernel ( $0\not=\eta^\pi\in\textup{Ker}\prn{\gI-\gT^\pi}$).
However, we find $\prn{\gI-\gT^\pi}$ is invertible on a subspace $\prn{\overline{M^0_{\FLip}}}^\gS$, with
\begin{equation*}
    M^0_{\FLip}:=\brc{\mu\text{ signed measure on }\prn{\brk{0,\frac{1}{1-\gamma}},\gB_0},\norm{\mu}_{\FLip}<\infty,\mu\prn{\brk{0,\frac{1}{1-\gamma}}}=0},    
\end{equation*}
which suffices for our analysis.

\begin{lemma}\label{Lemma_operator_invertible}
The operator $(\gI-\gT^\pi)$ is invertible on $\prn{\overline{M^0_{\FLip}}}^\gS$ and $\prn{\gI-\gT^\pi}^{-1}=\sum_{i=0}^\infty \prn{\gT^\pi}^i$.
\end{lemma}

Lemma~\ref{Lemma_operator_invertible} not only shows $(\gI-\gT^\pi)$ is invertible but constructs the inverse explicitly, thereby facilitating computational convenience.
Note that for $\nu\in\prn{M^0_{\FLip}}^\gS$,  it is not necessarily true that $\prn{\gI-\gT^\pi}^{-1}\nu\in\prn{M^0_{\FLip}}^\gS$ because the space $\prn{M^0_{\FLip}}^\gS$ are not complete.
Precisely, we have $\prn{\gI-\gT^\pi}^{-1}\nu\in\prn{\overline{M^0_{\FLip}}}^\gS$ that is a subspace of $\prn{\ell^\infty(\FLip)}^\gS$ for any $\nu\in \prn{M^0_{\FLip}}^\gS$.

To prove Lemma~\ref{Lemma_operator_invertible}, the main idea is to show the convergence of the Neumann series $\sum_{i=1}^\infty \prn{\gT^\pi}^i$.
% on $\prn{M^0_{\FLip}}^\gS$. 
% to show $\norm{\gT^\pi}_{\textup{op}}<1$ utilizing the contraction property of the distributional Bellman operator $\gT^\pi$.
% Given that the space $\prn{M^0_{\FLip}}^\gS$ is complete, the Neumann series is guaranteed to converge in $\prn{M^0_{\FLip}}^\gS$.
For any $\mu\in M^0_{\FLip}$, one has the decomposition $\mu=a_\mu(\mu_+-\mu_-)$ such that $a_\mu$ is a positive constant and $\mu_+,\mu_-$ are probability measures.
Thus $\norm{\mu}_{\FLip}=a_\mu W_1(\mu_+,\mu_-)$ and the convergence of Neumann series can be shown utilizing the contraction property of the distributional Bellman operator $\gT^\pi$.
One may refer to Appendix~\ref{Appendix_proof_asymp} for detailed proof.

Recall that we have previously demonstrated $\sqrt{n}\prn{\gI-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)\cweak \wtilde \GB^\pi$.
Thus our final step is to establish $\sqrt{n}(\hat\eta_n^\pi-\eta^\pi)\cweak \prn{\gI-\gT^\pi}^{-1}\wtilde \GB^\pi$.
This step can be accomplished as we always have $\sum_{s^\prime} Z_{s,a.s^\prime}=0$ for any state-action pair $(s,a)$, which implies $\wtilde\GB^\pi$ is also in $\prn{M^0_{\FLip}}^\gS$.

\paragraph{Weak Convergence in $\ell^\infty(\gF_{\mathsf{Ind}})$}

% Since the operator $\gT^\pi$ is no longer a contraction with respect to the $\KS$ metric (corresponding to $\norm{\cdot}_{\FInd}$), we need to add some restrictions on the normed vector space $ M_{\FInd}$ for convenience of our analysis.
% Concretely, we define
% \begin{equation*}
%     \wtilde M_{\FInd}:=\brc{\mu\text{ signed measure on }\prn{\brk{0,\frac{1}{1-\gamma}},\gB_0},\norm{\mu}_{\FInd}<\infty,\text{ $\mu$ has a density }}.
% \end{equation*}
% Here we say $\mu$ has a density if there exists some function $f$ supported on $\brk{0,\frac{1}{1-\gamma}}$ such that for any $B\in\gB_0$, $\mu(B)=\int_B f(x)dx$.
% $\wtilde M_{\FInd}$ is a subspace of $M_{\FInd}$ and both $\hat\eta_n^\pi$ and $\eta_n^\pi$ lie in $\prn{\wtilde M_{\FInd}}^\gS$ as long as Assumption~\ref{Assumption_reward_bounded_density} holds.
% Furthermore, it is straightforward to verify that $\what\gT^\pi\nu,\gT^\pi\nu\in \prn{\wtilde M_{\FInd}}^\gS$ as long as $\nu\in\prn{\wtilde M_{\FInd}}^\gS$.
$M_{\FInd}$ contains all probability measures supported on $\brk{0,\frac{1}{1-\gamma}}$.
As a result, the following decomposition is still valid with all relevant terms in $\prn{ M_{\FInd}}^\gS$.
\begin{equation*}
    \sqrt{n}\prn{\gI-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)=\underbrace{\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}_{(1)}+\underbrace{\sqrt{n}\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}_{(2)}.
\end{equation*}
We also have
\begin{lemma}\label{Lemma_convergence_difference_operator_Ind}
Let Assumption~\ref{Assumption_reward_bounded_density} hold.
For any $s\in\gS$, $\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}(s)$ converge weakly to the process $f\mapsto \wtilde\GB^\pi(s)f$ in $\ell^\infty(\FInd)$.
Here the random element $\wtilde\GB^\pi$ is defined as
    \begin{equation*}
        \wtilde\GB^\pi(s):=\sum_{a\in\gA}\pi(a\mid s)\sum_{s^\prime\in\gS} Z_{s,a,s^\prime}\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\ \forall s\in\gS,
    \end{equation*}
    where  $\prn{Z_{s,a,s^\prime}}_{s\in\gS,a\in\gA,s^\prime\in\gS}$ are zero-mean gaussians with 
    \begin{equation*}
    \cov(Z_{s_1,a_1,s_1^\prime},Z_{s_2,a_2,s_2^\prime})=\ind\brc{(s_1,a_1)=(s_2,a_2)}P(s_1^\prime\mid s_1,a_1)\prn{\ind\brc{s_1^\prime=s_2^\prime}-P(s_2^\prime\mid s_1,a_1)}.
    \end{equation*}
\end{lemma}
\begin{lemma}\label{Lemma_convergence_res_op1_Ind}
Let Assumption~\ref{Assumption_reward_bounded_density} hold.
For any $s\in\gS$, we have ${\norm{\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}(s)}_{\FInd}=o_P\prn{1}}$.
\end{lemma}

The proof strategy is similar to that of Lemma~\ref{Lemma_convergence_difference_operator} and Lemma~\ref{Lemma_convergence_res_op1}.
One may refer to Appendix~\ref{Appendix_proof_asymp} for detailed proof.

As before, the next step is to show $(\gT-\gT^\pi)$ is invertible on some space containing the signed measures of interest.
Specifically, let
\begin{equation*}
    M_{\FInd}^0:=\brc{\mu\text{ signed measure on }\prn{\brk{0,\frac{1}{1-\gamma}},\gB_0},\norm{\mu}_{\FLip}<\infty,\mu\prn{\brk{0,\frac{1}{1-\gamma}}}=0,\mu\text{ has bounded density.}}
\end{equation*}
Here we say $\mu$ has a density if there exists some function $f$ supported on $\brk{0,\frac{1}{1-\gamma}}$ such that for any $B\in\gB_0$, $\mu(B)=\int_B f(x)dx$.
The existence of bounded density allows us to control the $\norm{\cdot}_{\FInd}$ with $\norm{\cdot}_{\FLip}$.
When Assumption~\ref{Assumption_reward_bounded_density} is true, we always have $(\eta^\pi-\hat\eta_n^\pi)\in\prn{M_{\FInd}^0}^\gS$ and it is easy to verify $\gT^\pi\nu\in\prn{M_{\FInd}^0}^\gS$ as long as $\nu\in\prn{M_{\FInd}^0}^\gS$.

\begin{lemma}\label{Lemma_operator_invertible_Ind}
The operator $(\gI-\gT^\pi)$ is invertible on $\prn{\overline{M^0_{\FInd}}}^\gS$ and $\prn{\gI-\gT^\pi}^{-1}=\sum_{i=0}^\infty \prn{\gT^\pi}^i$.
\end{lemma}

Also for $\nu\in\prn{M^0_{\FInd}}^\gS$, $\prn{\gI-\gT^\pi}^{-1}\nu$ does not necessarily lie in $\prn{M^0_{\FInd}}^\gS$.
Instead, we have $\prn{\gI-\gT^\pi}^{-1}\nu\in\prn{\overline{M^0_{\FInd}}}^\gS$ that is a subspace of $\prn{\ell^\infty(\FInd)}^\gS$ for any $\nu\in \prn{M^0_{\FInd}}^\gS$.
The proof techniques are a combination of the proof of Lemma~\ref{Lemma_operator_invertible} and Proposition~\ref{Proposition_bound_KS_with_W1}.

Finally, we can obtain $\sqrt{n}(\hat\eta_n^\pi-\eta^\pi)\cweak \prn{\gI-\gT^\pi}^{-1}\wtilde \GB^\pi$ since $\wtilde \GB^\pi$ is guaranteed to lie in $\prn{M^0_{\FInd}}^\gS$.

==> non_asymp_old.tex <==
%\subsection{Main Results}
\subsection{Results on Non-asymptotic Analysis}\label{Section_non_asymp}

Our main results of non-asymptotic analysis is given in the following theorem.
\begin{theorem}\label{Theorem_bound_of_Wdist}
For any fixed policy $\pi$, %we have for 
there exists a universal constant $K$ such that
\begin{equation*} \EB\sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))\leq \frac{\gamma}{(1-\gamma)(1-\gamma^p)^{1/p}}\brk{\frac{K\abs{\gS}\log(\abs{\gS}\abs{\gA})}{n}}^{\frac{1}{2p}}.
\end{equation*}
And for any $\delta\in(0,1)$, with probability at least $1-\delta$, it holds that
\begin{equation*}
\sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))\leq\frac{\gamma}{(1-\gamma)(1-\gamma^p)^{1/p}}\brk{\frac{\max\prn{\abs{\gS},2\log\prn{2|\gS||\gA|/\delta}}}{n}}^{\frac{1}{2p}}.
\end{equation*}

\end{theorem}

To sum up, we show that $n=\wtilde{O}\prn{\frac{\abs{\gS}}{\epsilon^{2p}(1-\gamma)^{2p+2}}}$ suffices to ensure both $\EB\sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))\leq\epsilon$ and $\sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))\leq \epsilon$ with high probability, which implies a model-based distributional policy evaluation is sample-efficient.
We prove Theorem~\ref{Theorem_bound_of_Wdist} by explicitly constructing couplings between $\eta^\pi(s)$ and $\hat\eta_n^\pi(s)$ for $s\in\gS$.
A more detailed outline of proof can be found in Section~\ref{Subsection_proof_bound_of_Wdist}.

Compared with the $\wtilde{O}\prn{\frac{1}{(1-\gamma)^3\epsilon^2}}$ sample complexity bound for the model-based policy evaluation \citep{li2020breaking}, our sample complexity bound has an additional $\frac{|\gS|}{1-\gamma}$ factor (taking $p=1$).
We comment that  the problem of learning the distribution of returns is harder than the policy evaluation problem because one always has $\abs{V(s)-\what V(s)}\leq W_1(\eta^\pi(s),\hat\eta_n^\pi(s))$.
However, the factor of $|\gS|$ arises from controlling $\TV(P(\cdot\mid s,a)$ and $ \what P(\cdot\mid s,a))$, which may not be necessary.
We speculate the additional $|\gS|$ factor can be eliminated with more refined analysis techniques.

Under Assumption~\ref{Assumption_reward_bounded_density}, we also have the following bounds on the KS metric, which is a direct corollary of Theorem~\ref{Theorem_bound_of_Wdist} and Proposition~\ref{Proposition_bound_KS_with_W1}.

\begin{corollary}\label{Corollary_bound_on_KS}
    Under Assumption~\ref{Assumption_reward_bounded_density}, for any fixed policy $\pi$, we have for some universal constant $K$,
    \begin{equation*} \EB\sup_{s\in\gS}\KS(\hat\eta_n^\pi(s),\eta^\pi(s))\leq \sqrt{\frac{2C\gamma}{(1-\gamma)^2}}\brk{\frac{K\abs{\gS}\log(\abs{\gS}\abs{\gA})}{n}}^{\frac{1}{4}}.
\end{equation*}
    And for any $\delta\in(0,1)$, with probability at least $1-\delta$, then
\begin{equation*}
\sup_{s\in\gS}\KS(\hat\eta_n^\pi(s),\eta^\pi(s))\leq
\sqrt{\frac{2C\gamma}{(1-\gamma)^2}}\brk{\frac{\max\prn{\abs{\gS},2\log\prn{2|\gS||\gA|/\delta}}}{n}}^{\frac{1}{4}}.
\end{equation*}

\end{corollary}

\subsubsection{Analysis of Theorem~\ref{Theorem_bound_of_Wdist}}\label{Subsection_proof_bound_of_Wdist}

From a high-level viewpoint, our proof consists of three steps: for any fixed $s\in\gS$, we first construct $\kappa^\pi(s)$ as a coupling of $\eta^\pi(s)$ and $\hat\eta_n^\pi(s)$; then we bound $\EB_{\prn{G,\what G}\sim\kappa^\pi(s)}\abs{G-\what G}^p$ with $\max_{s\in\gS,a\in\gA}\TV\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}$; and the final step is to bound ${\max_{s\in\gS,a\in\gA}\TV\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}}$.
We elaborate on these three steps in the sequel.

\paragraph{Constructing the Coupling $\kappa^\pi(s)$}
Given an initial state $s\in\gS$, we will first construct two random elements $\tau^\pi(s)=\brc{\prn{S_t,A_t,R_t}_{t=0}^\infty},\hat\tau^\pi(s)=\brc{\prn{\what S_t,\what A_t,\what R_t}_{t=0}^\infty}$ such that their laws are the distribution of the trajectory induced by $(P,\pi,\gP_R)$ and $\prn{\what{P},\pi,\gP_R}$, respectively.
For some specific trajectory $\tau=\brc{\prn{s_t,a_t,r_t}_{t=0}^\infty}$, we slightly abuse the notation and define the return of the trajectory $\tau$ as $G(\tau)=\sum_{t=0}^\infty\gamma^t r_t$.
Let $\kappa^\pi(s)$ be the joint distribution of $\prn{G(\tau^\pi(s)),G(\hat\tau^\pi(s))}$, $\kappa^\pi(s)$ is a coupling of $(\eta^\pi(s),\hat\eta_n^\pi(s))$.

Now we go into detail about the construction of $\tau^\pi(s)$ and $\hat\tau^\pi(s)$.
We divide the time axis into two intervals: the aligned interval $I_1=\brc{0,...,T_0}$ and the independent interval $I_2=\NB-I_1$.
We say time $t$ is in the aligned interval if the two trajectories $\tau^\pi(s)$ and $\hat\tau^\pi(s)$ up to time t are all the same.
And $T_0+1$ is the time point when the two trajectories differ for the first time.
WLOG we let $0\in I_1$.
The intuition is that we wish the aligned interval can be as far as possible.
The longer the aligned interval is, the smaller the difference $\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}$ is.

When current time $t$ in the aligned interval, given the current state-action pair $(S_t,A_t)=(\what S_t,\what A_t)$, we sample the next state $S_{t+1}$ and $\what S_{t+1}$ via the following procedures.
Let 
\[{p=\sum_{s\in\gS}P(s\mid S_t,A_t)\wedge\what P(s\mid S_t,A_t)},\] 
where $a\wedge b:=\min(a,b)$.
We first flip a coin with the probability of heads equal to $p$.
If the coin comes up heads, then we sample a value $S^\prime$ according to the distribution $\mu_1(s)=\frac{P(s\mid S_t,A_t)\wedge\what P(s\mid S_t,A_t)}{p}$ and set $S_{t+1}=\what S_{t+1}=S^\prime$.
If the coin comes up tails, then we sample $S_{t+1}$ according to the distribution 
\begin{equation*}
    \mu_2(s)=\begin{cases}
        \frac{P(s\mid S_t,A_t)-\what P(s\mid S_t,A_t)}{1-p} &\text{if } P(s\mid S_t,A_t)>\what P(s\mid S_t,A_t)\\
        0 & \text{otherwise}\\
    \end{cases}
\end{equation*}
and sample $\what S_{t+1}$ independently according to the distribution 
\begin{equation*}
    \mu_3(s)=\begin{cases}
        \frac{\what P(s\mid S_t,A_t)- P(s\mid S_t,A_t)}{1-p} &\text{if } \what P(s\mid S_t,A_t)> P(s\mid S_t,A_t)\\
        0 & \text{otherwise}.
    \end{cases}
\end{equation*}
We adopt such a sample scheme to ensure that $\PB\prn{S_{t+1}\not=\what S_{t+1}}=\TV\prn{P(\cdot\mid S_t,A_t),\what P(\cdot\mid S_t,A_t)}$.
If $S_{t+1}=\what S_{t+1}$, $t+1$ is still in the aligned interval and sample $A_{t+1}=\what A_{t+1}\sim \pi(\cdot\mid S_{t+1})$, $R_{t+1}=\what R_{t+1}\sim \gP_R(S_{t+1},A_{t+1})$.
Otherwise, we have $t+1$ belongs to the independent interval and sample $A_{t+1}\sim \pi(\cdot\mid S_{t+1})$, $\what A_{t+1}\sim \pi\prn{\cdot\mid\what S_{t+1}}$, $R_{t+1}\sim \gP_R(S_{t+1},A_{t+1})$, $\what R_{t+1}\sim \gP_R\prn{\what S_{t+1},\what A_{t+1}}$ independently.

When the current time $t$ is in the independent interval, then we simply sample ${S_{t+1}\sim P\prn{\cdot\mid S_t,A_t}}$, $\what S_{t+1}\sim \what P\prn{\cdot\mid \what S_t,\what A_t}$, $A_{t+1}\sim \pi(\cdot\mid S_{t+1})$, $\what A_{t+1}\sim \pi\prn{\cdot\mid\what S_{t+1}}$, $R_{t+1}\sim \gP_R(S_{t+1},A_{t+1})$, ${\what R_{t+1}\sim \gP_R\prn{\what S_{t+1},\what A_{t+1}}}$  all independently.
It is straightforward to verify that the distribution laws of $\tau^\pi(s)$ and $\hat\tau^\pi(s)$ constructed by the rules described above are the distribution of the trajectory induced by $(P,\pi,\gP_R)$ and $\prn{\what{P},\pi,\gP_R}$, respectively.

\paragraph{Bounding $\EB\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p$ with $\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}$}

We write the event $E_t:=\brc{\forall i\leq t, \prn{S_i,A_i,R_i}=\prn{\what S_i,\what A_i,\what R_i}}$ representing $t$ is in the aligned interval.
For some trajectory $\tau=\brc{(s_t,a_t,r_t)_{t=0}^\infty}$, let $G_j(\tau):=\sum_{t=j}^\infty \gamma^{t-j}r_t$.
Noting that conditioned on event $E_j$, we have $\abs{G(\tau^\pi(s))-G(\hat \tau^\pi(s))}=\gamma^j\abs{G_j(\tau^\pi(s))-G_j(\hat \tau^\pi(s))}$.
We may form a partition of the sample space based on the sequence of events $E_1,E_2,\dots,E_N$ and get
\begin{equation*}
    \begin{aligned}
        \abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p
        &=\gamma^p\abs{G_1(\tau^\pi(s))-G_1(\hat\tau^\pi(s))}^p(\ind_{E_1}+\ind_{E_1^c})\\
        &\leq \gamma^p\abs{G_1(\tau^\pi(s))-G_1(\hat\tau^\pi(s))}^p\ind_{E_1}+\gamma^p\prn{\frac{1}{1-\gamma}}^p\ind_{E_1^c}\\
        &\leq \gamma^{pN}\abs{G_N(\tau^\pi(s))-G_N(\hat\tau^\pi(s))}^p\ind_{E_N}+\gamma^p\prn{\frac{1}{1-\gamma}}^p\sum_{j=1}^N \gamma^{p(j-1)}\ind_{E_{j-1}\cap E_j^c}\\
        &\leq \gamma^{pN}\prn{\frac{1}{1-\gamma}}^p+\gamma^p\prn{\frac{1}{1-\gamma}}^p\sum_{j=1}^N \gamma^{p(j-1)}\ind_{E_{j-1}\cap E_j^c}\\
        &=\prn{\frac{1}{1-\gamma}}^p\prn{\gamma^{pN}+\sum_{j=1}^N \gamma^{pj}\ind_{E_{j-1}\cap E_j^c}}.
    \end{aligned}
\end{equation*}
Then we have 
\begin{equation*}
    \begin{aligned}
        \EB_{\kappa^\pi(s)}\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p
        \leq \prn{\frac{1}{1-\gamma}}^p\brk{\gamma^{pN}+\sum_{j=1}^N\gamma^{pj}\kappa^\pi(s)\prn{E_{j-1}\cap E_j^c}}.
    \end{aligned}
\end{equation*}
Recall that $\kappa^\pi(s)$ is the coupling we construct in the previous step and
\begin{equation*}
    \begin{aligned}
        \kappa^\pi(s)\prn{E_{j-1}\cap E_j^c}\leq \kappa^\pi(s)\prn{E_{j-1}\mid E_j^c} \leq \max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}.
    \end{aligned}
\end{equation*}
Here the last inequality holds by the construction of $\kappa^\pi(s)$.
Consequently, we have
\begin{equation*}
    \begin{aligned}
        \EB_{\kappa^\pi(s)}\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p
        &\leq \prn{\frac{1}{1-\gamma}}^p\brk{\gamma^{pN}+\sum_{j=1}^N\gamma^{pj}\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}}\\
        &\leq \frac{\gamma^p\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}}{(1-\gamma)^p(1-\gamma^p)},
    \end{aligned}
\end{equation*}
where the last inequality holds since $N$ is arbitrarily chosen.

\paragraph{Bounding $\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}$} 
In our last step, we may get a bound of $\EB\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}$ and a high probability bound of $\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}$ by standards techniques in concentration of measures.
We state the bounds in the following two lemmas and the proofs are given in Appendix~\ref{Appendix_proof_non_asymp}.
\begin{lemma}\label{Lemma_bound_of_expected_TV} There exists a universal constant $K$ such that
    \begin{equation*}  \EB\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}\leq \sqrt{\frac{K\abs{\gS}\log\prn{\abs{\gS}\abs{\gA}}}{n}}.
    \end{equation*}
\end{lemma}
\begin{lemma}\label{Lemma_high_prob_bound_of_TV}
    For any $\delta\in(0,1)$, with probability at least $1-\delta$,
    \begin{equation*}  \max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}\leq \sqrt{\frac{\max\prn{\abs{\gS},2\log\prn{2|\gS||\gA|/\delta}}}{n}}.
    \end{equation*}
\end{lemma}

Then we put everything together and get that there exists a universal constant $K$ such that
\begin{equation*}
\begin{aligned}
    \EB\sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))&\leq\EB\sup_{s\in\gS} \brk{\EB_{\kappa^\pi(s)}\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p}^{\frac{1}{p}}\\
    &\leq \sup_{s\in\gS}\frac{\gamma\EB\brk{\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}}^{\frac{1}{p}}}{(1-\gamma)(1-\gamma^p)^{1/p}}\\
    &\leq\frac{\gamma}{(1-\gamma)(1-\gamma^p)^{1/p}}\brk{\frac{K\abs{\gS}\log(\abs{\gS}\abs{\gA})}{n}}^{\frac{1}{2p}}.
\end{aligned}
\end{equation*}
And for any $\delta\in(0,1)$, with probability at least $1-\delta$,
\begin{equation*}
\begin{aligned}
    \sup_{s\in\gS}W_p(\hat\eta_n^\pi(s),\eta^\pi(s))&\leq\sup_{s\in\gS} \brk{\EB_{\kappa^\pi(s)}\abs{G(\tau^\pi(s))-G(\hat\tau^\pi(s))}^p}^{\frac{1}{p}}\\
    &\leq \sup_{s\in\gS}\frac{\gamma\brk{\max_{s\in\gS,a\in\gA}\mathrm{TV}\prn{P(\cdot\mid s,a),\what P(\cdot\mid s,a)}}^{\frac{1}{p}}}{(1-\gamma)(1-\gamma^p)^{1/p}}\\
    &\leq\frac{\gamma}{(1-\gamma)(1-\gamma^p)^{1/p}}\brk{\frac{\max\prn{\abs{\gS},2\log\prn{2|\gS||\gA|/\delta}}}{n}}^{\frac{1}{2p}}.
\end{aligned}
\end{equation*}

==> proof_asymp_old.tex <==
\begin{proof}[Proof of Lemma~\ref{Lemma_convergence_difference_operator}]
For any $s\in\gS$, we have
\begin{equation*}
    \begin{aligned}
        \sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}(s)&=\sum_{a\in\gA}\pi(a\mid s)\sum_{s^\prime\in\gS} \sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a)\\
        &=\sum_{a\in\gA,s^\prime\in\gS}\brk{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}\brk{\pi(a\mid s)\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a)}
    \end{aligned}
\end{equation*}
    Thus the conclusion follows via the multivariate CLT and Lemma~\ref{Lemma_simple_weak_convergence}.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{Lemma_convergence_res_op1}]
    For any $s\in\gS$, we have
    \begin{equation*}
        \begin{aligned}
            &\norm{\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}(s)}_{\FLip}\\
            &=\norm{\sum_{a\in\gA,s^\prime\in\gS}\brk{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}\brk{\pi(a\mid s)\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}}_{\FLip}\\
            &\leq \norm{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}_1\sup_{a\in\gA,s^\prime\in\gS}\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FLip}.
        \end{aligned}
    \end{equation*}
    Since $\norm{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}_1$ is of the order $O_P(1)$, it suffices to show for any $s^\prime\in\gS, a\in\gA$, $\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FLip}=o_P(1)$.
    Noting that 
    \begin{equation*}
    \begin{aligned}
        &\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FLip}\\
        &=W_1\prn{\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)}.
    \end{aligned}
    \end{equation*}
    We claim that
    \begin{equation*}
    \begin{aligned}
        W_1\prn{\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)}\leq W_1\prn{\hat\eta_n^\pi(s^\prime),\eta^\pi(s^\prime)}.
    \end{aligned}
    \end{equation*}
    For simplicity of notations, we use $\hat\nu$ in short of $\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)$ and $\nu$ in short of $\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a)$.
    In fact, suppose two random variables $X\sim \eta^\pi(s^\prime)$, $Y\sim\hat\eta_n^\pi(s^\prime)$, and an independent random variable $R\sim \gP_R(dr\mid s,a)$, then $R+\gamma Y\sim \hat\nu$ and $R+\gamma X\sim \nu$.
    Then we have
    \begin{equation*}
    \begin{aligned}
        &W_1\prn{\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)}\\
        &=\inf_{W\sim \nu, Z\sim \hat \nu}\EB\abs{W-Z}\\
        &\leq \EB\abs{(R+\gamma X)-(R+\gamma Y)}\\
        &=\gamma\EB\abs{X-Y}.
    \end{aligned}
    \end{equation*}
    Our claim is true since $X$ and $Y$ are chosen arbitrarily.
    Our conclusion follows since by Theorem~\ref{Theorem_bound_of_Wdist} $W_1(\eta^\pi(s^\prime),\hat\eta^\pi_n(s^\prime))=o_P(1)$.
\end{proof}
% \begin{lemma}\label{Lemma_lip_space_Banach}
%     $\prn{M^0_{\FLip}}^\gS$ is a Banach space.
% \end{lemma}
\begin{proof}[Proof of Lemma~\ref{Lemma_operator_invertible}]
    It suffices to verify that the Neumann series $\sum_{i=0}^\infty\prn{\gT^\pi}^i$ converges in $\prn{M^0_{\FLip}}^\gS$.
    First, we claim for any $\nu\in \prn{M^0_{\FLip}}^\gS$, $\brc{\sum_{i=1}^k\prn{\gT^\pi}^i\nu,k=1,2,\dots}$ is a Cauchy sequence.
    WLOG, for any $\nu\in \prn{M^0_{\FLip}}^\gS$, $s\in\gS$, we may write $\nu=a_\nu(s)\prn{\nu_+(s)-\nu_-(s)}$, where $a_\nu(s)$ is a positive constant and $\nu_+(s),\nu_-(s)\in\Delta\prn{[0,\frac{1}{1-\gamma}]}$.
    Note that $\norm{\nu(s)}_{\FLip}=a_\nu(s) W_1(\nu_+(s),\nu_-(s))$ for any $s\in\gS$.
    For $k_1<k_2$, we have for any $s\in\gS$
    \begin{equation*}
        \begin{aligned}
            \norm{\sum_{i=k_1}^{k_2}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}&\leq\sum_{i=k_1}^{k_2}\norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}\\
            &=a_\nu(s)\sum_{i=k_1}^{k_2}W_1\prn{\brk{\prn{\gT^\pi}^i\nu_+}(s),\brk{\prn{\gT^\pi}^i\nu_-}(s)}\\
            &\leq a_\nu(s)\sum_{i=k_1}^{k_2}\gamma^i\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}\\
            &\leq \frac{\gamma^{k_1}a_\nu(s)\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}{1-\gamma}.
        \end{aligned}
    \end{equation*}
    The second last inequality is due to Proposition~\ref{Proposition_value_iteration_Wp}.
    Then we define $\nu_*$ such that for any $f\in\FLip$, $\nu_*(s)f:=\lim_{k\to\infty}\sum_{i=0}^k\brk{\prn{\gT^\pi}^i\nu}(s)f$. 
    $\nu_*$ is well-defined because $\brc{\sum_{i=1}^k\prn{\gT^\pi}^i\nu(s) f,k=1,2,\dots}$ is a Cauchy sequence in $\RB$ by similar arguments as above.
    As 
    \begin{equation*}
        \begin{aligned}
            \norm{\nu_*(s)-\sum_{i=0}^{k}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}
            &=\norm{\sum_{i=k}^{\infty}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}\\
            &\leq \sum_{i=k}^\infty \norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}\\
            &\leq \frac{\gamma^{k}a_\nu(s)\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}{1-\gamma},
        \end{aligned}
    \end{equation*}
    $\nu_*=
    \lim_{k\to\infty}\sum_{i=1}^k\prn{\gT^\pi}^i\nu$.
    % And our conclusion follows since $\nu_*\in \prn{M^0_{\FLip}}^\gS$ by that $\forall s\in\gS$,
    % \begin{equation*}
    % \begin{aligned}
    %     \norm{\nu_*(s)}_{\FLip}&\leq \sum_{i=0}^{\infty}\norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FLip}\\
    %     &\leq \frac{a_\nu\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}{1-\gamma}\\
    %     &<\infty.
    % \end{aligned}
    % \end{equation*}
    Apparently $\nu_*\in \prn{\overline{M^0_{\FLip}}}^\gS$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{Lemma_convergence_difference_operator_Ind}]
The proof is identical to that of Lemma~\ref{Lemma_convergence_difference_operator}.
For any $s\in\gS$, we have
\begin{equation*}
    \begin{aligned}
        \sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}\eta^\pi}(s)=\sum_{a\in\gA,s^\prime\in\gS}\brk{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}\brk{\pi(a\mid s)\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a)}
    \end{aligned}
\end{equation*}
    Thus the conclusion follows via the multivariate CLT and Lemma~\ref{Lemma_simple_weak_convergence}.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{Lemma_convergence_res_op1_Ind}]
    For any $s\in\gS$, we have
    \begin{equation*}
        \begin{aligned}
            &\norm{\sqrt{n}\brk{\prn{\what \gT_n^\pi-\gT^\pi}(\hat\eta_n^\pi-\eta^\pi)}(s)}_{\FInd}\\
            &=\norm{\sum_{a\in\gA,s^\prime\in\gS}\brk{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}\brk{\pi(a\mid s)\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}}_{\FInd}\\
            &\leq \norm{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}_1\sup_{a\in\gA,s^\prime\in\gS}\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FInd}.
        \end{aligned}
    \end{equation*}
    Since $\norm{\sqrt{n}\prn{\what P(s^\prime\mid s,a)-P(s^\prime\mid s,a)}}_1$ is of the order $O_P(1)$, it suffices to show for any $s^\prime\in\gS, a\in\gA$, $\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FInd}=o_P(1)$.
    Noting that 
    \begin{equation*}
    \begin{aligned}
        &\norm{\int_0^1 \brk{\prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)-\prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)}d\gP_R(dr\mid s,a)}_{\FInd}\\
        &=\KS\prn{\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)}.
    \end{aligned}
    \end{equation*}
    We claim that
    \begin{equation*}
    \begin{aligned}
        \KS\prn{\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a),\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)}\leq \KS\prn{\hat\eta_n^\pi(s^\prime),\eta^\pi(s^\prime)}.
    \end{aligned}
    \end{equation*}
    For simplicity of notations, we use $\hat\nu$ in short of $\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)d\gP_R(dr\mid s,a)$ and $\nu$ in short of $\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)d\gP_R(dr\mid s,a)$.
    In fact, for any $x\in\brk{0,\frac{1}{1-\gamma}}$,
    \begin{equation*}
    \begin{aligned}
        \abs{\hat\nu([0,x])-\nu([0,x])}&=\abs{\int_0^1 \prn{b_{r,\gamma}}_\#\hat\eta_n^\pi(s^\prime)([0,x])d\gP_R(dr\mid s,a)-\int_0^1 \prn{b_{r,\gamma}}_\#\eta^\pi(s^\prime)([0,x])d\gP_R(dr\mid s,a)}\\
        &=\abs{\int_0^1 \hat\eta_n^\pi(s^\prime)\prn{\brk{0,\frac{x-r}{\gamma}}}d\gP_R(dr\mid s,a)-\int_0^1 \eta^\pi(s^\prime)\prn{\brk{0,\frac{x-r}{\gamma}}}d\gP_R(dr\mid s,a)}\\
        &\leq \KS\prn{\hat\eta_n^\pi(s^\prime),\eta^\pi(s^\prime)}.
    \end{aligned}
    \end{equation*}
    Our claim is true since $x$ is chosen arbitrarily.
    Our conclusion follows since by Corollary~\ref{Corollary_bound_on_KS} $KS(\eta^\pi(s^\prime),\hat\eta^\pi_n(s^\prime))=o_P(1)$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{Lemma_operator_invertible_Ind}]
    It suffices to verify that the Neumann series $\sum_{i=0}^\infty\prn{\gT^\pi}^i$ converges in $\prn{M^0_{\FInd}}^\gS$.
    First, we claim for any $\nu\in \prn{M^0_{\FInd}}^\gS$, $\brc{\sum_{i=1}^k\prn{\gT^\pi}^i\nu,k=1,2,\dots}$ is a Cauchy sequence.
    WLOG, for any $\nu\in \prn{M^0_{\FInd}}^\gS$, $s\in\gS$, we may write $\nu=a_\nu(s)\prn{\nu_+(s)-\nu_-(s)}$, where $a_\nu(s)$ is a positive constant and $\nu_+(s),\nu_-(s)\in\Delta\prn{[0,\frac{1}{1-\gamma}]}$.
    Note that $\norm{\nu(s)}_{\FInd}=a_\nu(s) \KS(\nu_+(s),\nu_-(s))$ for any $s\in\gS$.
    There also exists a positive constant $C_\nu$ such that suppose for any $s\in\gS$, both $\nu_+(s)$ and $\nu_-(s)$ have a density bounded by $C_\nu$.
    For $k_1<k_2$, we have for any $s\in\gS$
    \begin{equation*}
        \begin{aligned}
            \norm{\sum_{i=k_1}^{k_2}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}&\leq\sum_{i=k_1}^{k_2}\norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}\\
            &=a_\nu(s)\sum_{i=k_1}^{k_2}\KS\prn{\brk{\prn{\gT^\pi}^i\nu_+}(s),\brk{\prn{\gT^\pi}^i\nu_-}(s)}\\
            &\leq a_\nu(s)\sum_{i=k_1}^{k_2}\sqrt{2C_\nu W_1\prn{\prn{\gT^\pi}^i\nu_+(s),\prn{\gT^\pi}^i\nu_-(s)}}\\
            &\leq a_\nu(s)\sum_{i=k_1}^{k_2}\sqrt{2C_\nu\gamma^i\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}\\
            &\leq \frac{\gamma^{k_1/2}a_\nu(s)\sqrt{2C_\nu\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}}{1-\sqrt{\gamma}}.
        \end{aligned}
    \end{equation*}
    The second inequality is by Proposition~\ref{Proposition_bound_KS_with_W1} and
    the third inequality is due to Proposition~\ref{Proposition_value_iteration_Wp}.
    Then we define $\nu_*$ such that for any $f\in\FLip$, $\nu_*(s)f:=\lim_{k\to\infty}\sum_{i=0}^k\brk{\prn{\gT^\pi}^i\nu}(s)f$. 
    $\nu_*$ is well-defined because $\brc{\sum_{i=1}^k\prn{\gT^\pi}^i\nu(s) f,k=1,2,\dots}$ is a Cauchy sequence in $\RB$ by similar arguments as above.
    As 
    \begin{equation*}
        \begin{aligned}
            \norm{\nu_*(s)-\sum_{i=0}^{k}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}
            &=\norm{\sum_{i=k}^{\infty}\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}\\
            &\leq \sum_{i=k}^\infty \norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}\\
            &\leq \frac{\gamma^{k/2}a_\nu(s)\sqrt{2C_\nu\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}}{1-\sqrt{\gamma}},
        \end{aligned}
    \end{equation*}
    $\nu_*=
    \lim_{k\to\infty}\sum_{i=1}^k\prn{\gT^\pi}^i\nu$.
    Apparently $\nu_*\in \prn{\overline{M^0_{\FInd}}}^\gS$.
%     $\forall s\in\gS$,
%     \begin{equation*}
%     \begin{aligned}
%         \norm{\nu_*(s)}_{\FInd}&\leq \sum_{i=0}^{\infty}\norm{\brk{\prn{\gT^\pi}^i\nu}(s)}_{\FInd}\\
%         &\leq \frac{a_\nu\sup_{s\in\gS}W_1\prn{\nu_+(s),\nu_-(s)}}{1-\gamma}\\
%         &<\infty.
%     \end{aligned}
%     \end{equation*}
%     To show $\nu_*$ has bounded density, it suffices to demonstrate the distribution function $F(x)=\nu_*(s)([0,x])$ is Lipschitz.
%     Note that for any $s\in\gS$, and $x_1,x_2\in\brk{0,\frac{1}{1-\gamma}}$, $x_1<x_2$,
%     \begin{equation*}
%         sss
%     \end{equation*}
%     Therefore,
%     \begin{equation*}
%         \abs{F(x_1)-F(x_2)}=\abs{\sum_{i=0}^\infty \brk{\prn{\gT^\pi}^i\nu}(s)([x_1,x_2])}
%     \end{equation*}
\end{proof}

